Springboard, Roadblock or "Crutch"?: How Transgender Users Leverage Voice Changers for Gender Presentation in Social Virtual Reality

Social virtual reality (VR) serves as a vital platform for transgender individuals to explore their identities through avatars and foster personal connections within online communities. However, it presents a challenge: the disconnect between avatar embodiment and voice representation, often leading to misgendering and harassment. Prior research acknowledges this issue but overlooks the potential solution of voice changers. We interviewed 13 transgender and gender-nonconforming users of social VR platforms, focusing on their experiences with and without voice changers. We found that using a voice changer not only reduces voice-related harassment, but also allows them to experience gender euphoria through both hearing their modified voice and the reactions of others to their modified voice, motivating them to pursue voice training and medication to achieve desired voices. Furthermore, we identified the technical barriers to current voice changer technology and potential improvements to alleviate the problems that transgender and gender-nonconforming users face.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> sections/tables/demographics.tex <==
\begin{table*}[h!]
    \footnotesize
    \centering
    \caption{Participants' demographics, social VR experiences, and voice changer experiences.}
    %\begin{tabular}{|c|c|c|c|c|c|c|c|}
    \begin{center}
    \begin{tabular}{p{1.1cm}p{0.3cm}p{1.5cm}p{5cm}p{3cm}p{2cm}p{2cm}}
    \toprule
    \textbf{ID} & \textbf{Age} & \textbf{Race/Ethnicity} & \textbf{Gender Identity} & \textbf{Social VR Experience} & \textbf{Voice Changer Experience} & \textbf{Voice Changer}\\
    \midrule
    P1 (pilot) & 37 & unknown & gender non-conforming & past experience & N/A & N/A \\
    P2 & 53 & caucasian & transgender female & 4-7 hours 4 days/week & present & Voicemod \\
    P3 & 28 & caucasian & agender & 3-6 hours, 5 days/week & present & Voicemod/Clownfish \\
    P4 & 32 & hispanic & transgender female & N/A & past & Clownfish \\
    P5 & 20 & caucasian & gender-nonconforming transmasc  & evenings, 2-3 days/week & present & Voicemod Pro \\
    P6 & 25 & caucasian & transgender female & weekly & present & Clownfish \\
    P7 & 22 & caucasian & transgender female & 6-12 hours/week & present & Clownfish \\
    P8 & 18 & brazilian & gender non-conforming transgender female & 2-3 hours daily & present & SuperVoiceChanger \\
    P9 & 36 & caucasian & transgender female & 1-3 hours daily & past & Clownfish/MorphVOX Junior \\
    P10 & 41 & caucasian & gender-nonconforming transgender female & variable & present & Voicemod Persona \\
    P11 & 30 & caucasian & transgender female & N/A & present & Voicemod \\
    P12 & 42 & caucasian & transgender female & limited & present & Voicemod Pro \\
    P13 & 31 & mixed & gender-nonconforming transmasc & 2-8 hours/week & past & MorphVOX Pro \\
    P14 & 34 & caucasian & transgender female & 4-9 hours/week & past & MorphVOX Junior \\
    \bottomrule
    \end{tabular}
    \end{center}
    \label{tab:participants_demographics}
\end{table*}

==> sections/tables/demographics_1.tex <==
\begin{table*}[h!]
    \footnotesize
    \centering
    \caption{Participant demographics \yuhang{ANSWERED: inconsistency in capitalization; the table also needs to be marked with color}}
\begin{center}
\begin{tabular}{p{1.5cm}p{1cm}p{2cm}p{2.5cm}p{2cm}p{1.5cm}p{1cm}p{2.5cm}}
\toprule
\textbf{Participant} & \textbf{Age} & \textbf{Race/Ethnicity} & \added{\textbf{Recruiting Avenue}} & \added{\textbf{Location}} & \textbf{Gender} & \added{\textbf{GNC}} & \added{\textbf{Transition Direction}} \\
\midrule
%pilot removedd
P1 & 53 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
P2 & 28 & Caucasian & \added{Flyer} & \added{United States} & Agender & \added{Yes} & \added{N/A} \\
P3 & 32 & Hispanic & \added{Discord} & \added{Brazil} & Female & \added{No} & \added{Transfeminine} \\
P4 & 20 & Caucasian & \added{Discord} & \added{United States} & Nonbinary & \added{Yes} & \added{Transmasculine} \\
P5 & 25 & Caucasian & \added{Discord} & \added{Germany} & Female & \added{No} & \added{Transfeminine} \\
P6 & 22 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
P7 & 18 & Brazilian & \added{Discord} & \added{Brazil} & Female & \added{Yes} & \added{Transfeminine} \\
P8 & 36 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
P9 & 41 & Caucasian & \added{Discord} & \added{United States} & Female & \added{Yes} & \added{Transfeminine} \\
P10 & 30 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
P11 & 42 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
P12 & 31 & Mixed & \added{Discord} & \added{United States} & Nonbinary & \added{Yes} & \added{Transmasculine} \\
P13 & 34 & Caucasian & \added{Discord} & \added{United States} & Female & \added{No} & \added{Transfeminine} \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:participants_demographics_1}
\end{table*}
